StylePredict: Machine Theory of Mind for Human Driver Behavior From Trajectories

Studies have shown that autonomous vehicles (AVs) behave conservatively in a traffic environment composed of human drivers and do not adapt to local conditions and socio-cultural norms. It is known that socially aware AVs can be designed if there exist a mechanism to understand the behaviors of human drivers. We present a notion of Machine Theory of Mind (M-ToM) to infer the behaviors of human drivers by observing the trajectory of their vehicles. Our M-ToM approach, called StylePredict, is based on trajectory analysis of vehicles, which has been investigated in robotics and computer vision. StylePredict mimics human ToM to infer driver behaviors, or styles, using a computational mapping between the extracted trajectory of a vehicle in traffic and the driver behaviors using graph-theoretic techniques, including spectral analysis and centrality functions. We use StylePredict to analyze driver behavior in different cultures in the USA, China, India, and Singapore, based on traffic density, heterogeneity, and conformity to traffic rules and observe an inverse correlation between longitudinal (overspeeding) and lateral (overtaking, lane-changes) driving styles.

==> Sections/0-abstract.tex <==
\begin{abstract}
% What is the problem? 

Studies have shown that autonomous vehicles (AVs) behave conservatively in a traffic environment composed of human drivers and do not adapt to local conditions and socio-cultural norms. It is known that socially aware AVs can be designed if there exist a mechanism to understand the behaviors of human drivers. We present a notion of Machine Theory of Mind (M-ToM) to infer the behaviors of human drivers by observing the trajectory of their vehicles. Our M-ToM approach, called \textit{StylePredict}, is based on trajectory analysis of vehicles, which has been investigated in robotics and computer vision. StylePredict mimics human ToM to infer driver behaviors, or styles, using a computational mapping between the extracted trajectory of a vehicle in traffic and the driver behaviors using graph-theoretic techniques, including spectral analysis and centrality functions. We use StylePredict to analyze driver behavior in different cultures in the USA, China, India, and Singapore, based on traffic density, heterogeneity, and conformity to traffic rules and observe an inverse correlation between longitudinal (overspeeding) and lateral (overtaking, lane-changes) driving styles. 




% From our analysis, we found that the intensity of longitudinal driving styles such as overspeeding is higher in more populated regions like India, lateral styles such as weaving and overtaking are more prominent in regions where drivers do not obey traffic rules, and that two-wheelers are more likely to overtake and weave through traffic in any region.


% CAN YOU PRESENT SOME NEW INSIGHTS ABOUT BEHAVIOR ANALYSIS IN DIFFERENT CULTURES BASED ON GRAPH-BASED TECHNIQUES: THE GOAL IS TO CONVEY THAT YOU WERE ABLE TO PERFORM THIS ANALYSIS OR CHARACTERISTICS BASED ON YOUR ANALYSIS
%our analysis suggests that the heterogeneity and population density of a region affects the frequency and the type of driver behavior in that region. We evaluate StylePredict in both simulated and real-world traffic environments, and use the Time Deviation Error (TDE) metric to measure the accuracy.

% We use centrality functions as a formal metric to distinguish between aggressive and conservative behaviors of all human drivers in a traffic video. Furthermore, we use spectral analysis to show that StylePredict is robust to noise in the sensor data. We use the Time Deviation Error (TDE) metric to evaluate StylePredict on both simulated and real-world traffic. Finally, we use StylePredict to study traffic in the USA, China, India, and Singapore, and our analysis suggests that the heterogeneity and population density of a region affects the frequency and the type of driver behavior in that region.
\end{abstract}

==> Sections/2-def.tex <==
% \section*{Modeling Traffic Through Traffic-Graphs}
\section{A Graph Theoretic Formulation of Driver Behavior }

\paragraph{Definition} The definition of driving behavior has not been consistent in the social traffic psychology literature. In their review paper on driving behavior research, Sagberg et al.~\cite{sagberg2015review} isolate the common elements from different definitions to summarize driving behavior as -- A global driving style that is identified through one or more specific indicators.

\paragraph{Categorization} A vehicle may be assigned a global driving style that is composed of one or more specific indicators. A global driving style refer to a generalized style of driving. For example, aggressive driving is a global style and is composed of specific indicators such as overspeeding, weaving through traffic, tailgating and so on. Conservative driving is another global style that may be composed of specific indicators such as driving at a uniform speed, braking often etc. Additional global styles can be found in Figure 2 of~\cite{sagberg2015review}. 

\paragraph{Measurement} Many studies on driving behavior research have measured driving behavior by assigning a behavior label to a vehicle according to a scale~\cite{taubman2004multidimensional,ishibashi2007indices}. However, these scales are known to contain bias~\cite{sagberg2015review}. More importantly, many parameters used to define these scales cannot be observed in realtime. Instead, the Social Intuition model characterizes driving behavior by explicitly modeling specific indicators to identify global driving styles. 



==> Sections/6-culture.tex <==
\section{Social Intuition in Different Cultures}
\label{sec: culture}
The traffic conditions differ significantly across geographic regions. For instance, the traffic is more regulated and ordered in western countries such as the U.S. Traffic in Asian countries such as India is more dense and vehicles do not conform to lane-driving. Such differences also contribute to different driving behaviors.

The Social Intuition model is not affected by differences in traffic conditions caused by geographical regions. We show that while the range of the centralities changes, aggressive vehicles are still associated with high centrality values while conservative vehicles remain associated with low centrality values.

The change in range of the centralities, however, has some implications. As vehicles in developed western countries, such as the U.S., typically observe traffic rules and so drive uniformly, differences in driving behavior are more imperceptible. Consequently, a vehicle in U.S. traffic having the highest centrality may not be subjectively classified as an aggressive vehicle by human standards.

\input{algorithm/algo2}

\input{img/qualitative}
